The dog-and-rabbit chase problem

The dog-and-rabbit chase problem is a classical problem that illustrates the concepts of elementary kinematics and, therefore, can be used in introductory mechanics teaching. By dealing with the relative motion, the problem naturally requires solving elementary differential equations and stimulates students to learn mathematics. The efficiency of the approach we adopt is emphasized by extending the class of problems that can be solved by applying it.

==> rrp_mathdefs.tex <==
%\newcommand{\opL}{\mathfrak{L}}
%\newcommand{\opN}{\mathfrak{N}}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

\newcommand{\ddiv}{\ensuremath{\mathop{\operator@font div}\nolimits}}
\newcommand{\grad}{\ensuremath{\mathop{\operator@font grad}\nolimits}}
\newcommand{\artanh}{\ensuremath{\mathop{\operator@font artanh}\nolimits}}
\newcommand{\sech}{\ensuremath{\mathop{\operator@font sech}\nolimits}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}

\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%

